Privacy Regularization: Joint Privacy-Utility Optimization in Language Models

Neural language models are known to have a high capacity for memorization of training samples. This may have serious privacy implications when training models on user content such as email correspondence. Differential privacy (DP), a popular choice to train models with privacy guarantees, comes with significant costs in terms of utility degradation and disparate impact on subgroups of users. In this work, we introduce two privacy-preserving regularization methods for training language models that enable joint optimization of utility and privacy through (1) the use of a discriminator and (2) the inclusion of a triplet-loss term. We compare our methods with DP through extensive evaluation. We show the advantages of our regularizers with favorable utility-privacy trade-off, faster training with the ability to tap into existing optimization approaches, and ensuring uniform treatment of under-represented subgroups.

==> body/related.tex <==
%\vspace{-1ex}
\section{Related Work}

It has been long recognized that training machine learning models on datasets containing personal data comes with privacy issues. Many recent research efforts examine the vulnerability of such models or propose mitigations. 

Our work is closely related to \cite{coavoux18} and \cite{li2018}. In \cite{coavoux18}, the authors consider an attack model where an attacker eavesdrops on the hidden representations corresponding to an input and tries to recover information about the input text, such as gender or demographic information about the author of a text. They use adversarial training as mitigation to reduce the performance of an attacker and the setting is considered for the privacy of a text provided by a user at inference-time. In contrast, our goal is to prevent the model from learning sensitive information in the training set and we use adversarial training in this framework. On the other hand, \cite{li2018} use adversarial training to protect private author attributes such as age, gender, and location applied to part-of-speech tagging and sentiment analysis. Removal of such attributes can provide better generalisation, and can provide better privacy especially when latent representations of the data are shared for processing. We note that this is orthogonal to our work in terms of privacy as our goal is to protect sensitive information in the training set being encoded by the model. Our work is also related to \cite{olympus} where an obfuscation mechanism is applied to sensor data to limit the risk of disclosing private user information. The setting is considered where user data is fed to third party apps. We instead investigate the setting of a model training with privacy-utility consideration.

The {exposure} metric is introduced in \cite{carlini19} to quantitatively assess the unintentional memorization phenomenon occurring in generative sequence models. We use this metric to evaluate the mitigation effects of our approaches and extend it with an additional sequence extraction metric to evaluate the privacy risks in realistic settings. 

Prior work has studied the vulnerability of machine learning models to membership inference attack \cite{shokri17, yeom18, song19, long18, truex18}. The goal is to determine if a particular data record (or more generally data of a given user) belongs to the training set of the model. The key point making such attacks successful is that the models behave differently on the data records of their training set compared to the unseen data (i.e. performing better, predicting more confidently or providing better ranks etc.). This is also an orthogonal line of work to our paper as our main interest is not mitigating towards reducing this behavioral difference. 
%We are mainly interested in a well-performing language model that does not learn sensitive information found in the training dataset.

The main framework with theoretical guarantees for model privacy is the application of differential privacy (DP)~\cite{dwork2011differential} to model training. DP makes provable guarantees about the privacy of a stochastic function of a given dataset. Differentially private stochastic gradient descent (DP-SGD) has been developed and applied to deep learning \cite{song13, abadi2016deep}. While DP-SGD is a promising avenue for private model training, further research is needed to determine that DP-SGD can yield acceptable privacy-utility trade-offs as current deep learning models require high privacy budgets to achieve reasonable utility losses and this can in turn lead to successful privacy attacks \cite{jayaraman19, wang18, disparate}, undermining the efficacy of the privacy mechanism.
